Hypergraph $p$-Laplacians and Scale Spaces

This paper introduces gradient, adjoint, and $p$-Laplacian definitions for oriented hypergraphs as well as differential and averaging operators for unoriented hypergraphs. These definitions are used to define gradient flows in the form of diffusion equations with applications in modelling group dynamics and information flow in social networks as well as performing local and non-local image processing.

==> 3_diff_new.tex <==
\section{Differential operators on hypergraphs}
\label{diffOperators}

\af{The following section introduces first and higher order differential operators, both for unoriented and oriented hypergraphs.}

\subsection{First-order differential operators on oriented hypergraphs}

Instead of a vertex gradient, we define an averaging operator.

\begin{definition}[\textbf{Vertex averaging operator $\nabla_v$}]\label{Hnabla_v}
	For an unoriented hypergraph $UH = \left(\mathcal{V}, \mathcal{E}_H\right)$ with vertex weight functions $w_I$ and $w_G$ and hyperedge weight function $W_G$, we define the vertex gradient operator $\nabla_v$ with parameters $\alpha, \gamma, \kappa \in \mathbb{R}$ as:
	{\small\begin{equation*}
		\nabla_v: ~ \mathcal{H}\left(\mathcal{V}\right) \longrightarrow \mathcal{H}\left(\mathcal{E}_H\right) \quad f \longmapsto \nabla_v f
	\end{equation*}
        \begin{equation*}
            \nabla_v f: ~ \mathcal{E}_H \longrightarrow \mathbb{R} \quad e_q \longmapsto \nabla_v f \left(e_q\right) = 
        \end{equation*}
	\begin{equation}
		W_G \left(e_q\right)^\gamma \sum_{v_i \in \mathcal{V}} \delta\left(v_i, e_q\right) \frac{w_I\left(v_i\right)^\alpha w_G\left(v_i\right)^\kappa}{\left\lvert e_q\right\rvert} f\left(v_i\right).
	\end{equation}}
\end{definition}



\begin{definition}[\textbf{Vertex adjoint operator $\nabla^*_v$}]\label{Hnabla^*_v} 
	For an unoriented hypergraph $UH = \left(\mathcal{V}, \mathcal{E}_H\right)$ with vertex weight function $w_G$ and hyperedge weight functions $W_I$ and $W_G$, the vertex adjoint operator $\nabla^*_v$ with parameters $\beta, \gamma, \kappa \in \mathbb{R}$ is given by:
	{\small\begin{equation*}
		\nabla^*_v: ~ \mathcal{H}\left(\mathcal{E}_H\right) \longrightarrow \mathcal{H}\left(\mathcal{V}\right) \quad F \longmapsto \nabla^*_v F
	\end{equation*}
        \begin{equation*}
            \nabla^*_v F: ~ \mathcal{V} \longrightarrow \mathbb{R} \quad v_i \longmapsto \nabla^*_v F \left(v_i\right) =
        \end{equation*}
	\begin{equation}
		\sum_{e_q \in \mathcal{E}_H} \delta\left(v_i, e_q\right) \frac{w_G \left(v_i\right)^\kappa}{\left\lvert e_q\right\rvert} W_I \left(e_q\right)^\beta W_G \left(e_q\right)^\gamma F\left(e_q\right).
	\end{equation}}
\end{definition}

\begin{definition}[\textbf{Vertex divergence operator $\mathrm{div}_v$ ???}]\label{Hdiv_v}
	For an unoriented hypergraph $UH = \left(\mathcal{V}, \mathcal{E}_H\right)$ with vertex weight function $w_G$ and hyperedge weight functions $W_I$ and $W_G$, the vertex divergence operator $\mathrm{div}_v$ with parameters $\beta, \gamma, \kappa \in \mathbb{R}$ is given by:
	{\small\begin{equation*}
		\mathrm{div}_v: ~ \mathcal{H}\left(\mathcal{E}_H\right) \longrightarrow \mathcal{H}\left(\mathcal{V}\right) \quad F \longmapsto \mathrm{div}_v F
	\end{equation*}
        \begin{equation*}
            \mathrm{div}_v F: ~ \mathcal{V} \longrightarrow \mathbb{R} \quad v_i \longmapsto \mathrm{div}_v F \left(v_i\right) =
        \end{equation*}
	\begin{equation}
		\nabla^*_v F \left(v_i\right) = \sum_{e_q \in \mathcal{E}_H} \delta\left(v_i, e_q\right) \frac{w_G \left(v_i\right)^\kappa}{\left\lvert e_q\right\rvert} W_I \left(e_q\right)^\beta W_G \left(e_q\right)^\gamma F\left(e_q\right).
	\end{equation}}
\end{definition}

==> scraps.tex <==
\begin{definition}[\textbf{Vertex averaging operator $\nabla_v$}]\label{Hnabla_v}
	For an unoriented hypergraph $UH = \left(\mathcal{V}, \mathcal{E}_H\right)$ with vertex weight functions $w_I$ and $w_G$ and hyperedge weight function $W_G$, we define the vertex gradient operator $\nabla_v$ with parameters $\alpha, \gamma, \kappa \in \mathbb{R}$ as:
	{\small\begin{equation*}
		\nabla_v: ~ \mathcal{H}\left(\mathcal{V}\right) \longrightarrow \mathcal{H}\left(\mathcal{E}_H\right) \quad f \longmapsto \nabla_v f
	\end{equation*}
        \begin{equation*}
            \nabla_v f: ~ \mathcal{E}_H \longrightarrow \mathbb{R} \quad e_q \longmapsto \nabla_v f \left(e_q\right) = 
        \end{equation*}
	\begin{equation}
		W_G \left(e_q\right)^\gamma \sum_{v_i \in \mathcal{V}} \delta\left(v_i, e_q\right) \frac{w_I\left(v_i\right)^\alpha w_G\left(v_i\right)^\kappa}{\left\lvert e_q\right\rvert} f\left(v_i\right).
	\end{equation}}
\end{definition}



\begin{definition}[\textbf{Vertex adjoint operator $\nabla^*_v$}]\label{Hnabla^*_v} 
	For an unoriented hypergraph $UH = \left(\mathcal{V}, \mathcal{E}_H\right)$ with vertex weight function $w_G$ and hyperedge weight functions $W_I$ and $W_G$, the vertex adjoint operator $\nabla^*_v$ with parameters $\beta, \gamma, \kappa \in \mathbb{R}$ is given by:
	{\small\begin{equation*}
		\nabla^*_v: ~ \mathcal{H}\left(\mathcal{E}_H\right) \longrightarrow \mathcal{H}\left(\mathcal{V}\right) \quad F \longmapsto \nabla^*_v F
	\end{equation*}
        \begin{equation*}
            \nabla^*_v F: ~ \mathcal{V} \longrightarrow \mathbb{R} \quad v_i \longmapsto \nabla^*_v F \left(v_i\right) =
        \end{equation*}
	\begin{equation}
		\sum_{e_q \in \mathcal{E}_H} \delta\left(v_i, e_q\right) \frac{w_G \left(v_i\right)^\kappa}{\left\lvert e_q\right\rvert} W_I \left(e_q\right)^\beta W_G \left(e_q\right)^\gamma F\left(e_q\right).
	\end{equation}}
\end{definition}

\begin{definition}[\textbf{Vertex divergence operator $\mathrm{div}_v$ ???}]\label{Hdiv_v}
	For an unoriented hypergraph $UH = \left(\mathcal{V}, \mathcal{E}_H\right)$ with vertex weight function $w_G$ and hyperedge weight functions $W_I$ and $W_G$, the vertex divergence operator $\mathrm{div}_v$ with parameters $\beta, \gamma, \kappa \in \mathbb{R}$ is given by:
	{\small\begin{equation*}
		\mathrm{div}_v: ~ \mathcal{H}\left(\mathcal{E}_H\right) \longrightarrow \mathcal{H}\left(\mathcal{V}\right) \quad F \longmapsto \mathrm{div}_v F
	\end{equation*}
        \begin{equation*}
            \mathrm{div}_v F: ~ \mathcal{V} \longrightarrow \mathbb{R} \quad v_i \longmapsto \mathrm{div}_v F \left(v_i\right) =
        \end{equation*}
	\begin{equation}
		\nabla^*_v F \left(v_i\right) = \sum_{e_q \in \mathcal{E}_H} \delta\left(v_i, e_q\right) \frac{w_G \left(v_i\right)^\kappa}{\left\lvert e_q\right\rvert} W_I \left(e_q\right)^\beta W_G \left(e_q\right)^\gamma F\left(e_q\right).
	\end{equation}}
\end{definition}

\begin{theorem}[\textbf{Connection vertex gradient $\nabla_v$ and vertex adjoint $\nabla^*_v$}]\label{Hvertexgradadj} \ \\
	For a weighted unoriented hypergraph $UH = \left(\mathcal{V}, \mathcal{E}_H, w, W\right)$, the vertex adjoint operator $\nabla^*_v$ fulfills the equality
	\begin{equation}
		{\langle G, \nabla_v f \rangle}_{\mathcal{H}\left(\mathcal{E}_H\right)} = {\langle f, \nabla^*_v G \rangle}_{\mathcal{H}\left(\mathcal{V}\right)}
	\end{equation}
	for all vertex functions $f \in \mathcal{H}\left(\mathcal{V}\right)$ and all hyperedge functions $G \in \mathcal{H}\left(\mathcal{E}_H\right)$.\\
\end{theorem}

\begin{proof}\ \\
	Given a weighted unoriented hypergraph $UH = \left(\mathcal{V}, \mathcal{E}_H, w, W\right)$, a vertex function $f \in \mathcal{H}\left(\mathcal{V}\right)$ and a hyperedge function $G \in \mathcal{H}\left(\mathcal{E}_H\right)$, using the definitions of the inner product of $\mathcal{H}\left(\mathcal{E}_H\right)$ and $\mathcal{H}\left(\mathcal{V}\right)$ together with the vertex gradient operator $\nabla_v$ yields the following:\\
 
	$\begin{aligned}[t]
		{\langle G, \nabla_v f \rangle}_{\mathcal{H}\left(\mathcal{E}_H\right)} = & \sum_{e_q \in \mathcal{E}_H} W_I \left(e_q\right)^\beta G\left(e_q\right) \nabla_v f \left(e_q\right) &\\
	\end{aligned}$\\
	$\begin{aligned}[t]
		= & \sum_{e_q \in \mathcal{E}_H} W_I \left(e_q\right)^\beta G\left(e_q\right) W_G \left(e_q\right)^\gamma \sum_{v_i \in \mathcal{V}} \delta\left(v_i, e_q\right) \frac{w_I\left(v_i\right)^\alpha w_G\left(v_i\right)^\kappa}{\left\lvert e_q\right\rvert} f\left(v_i\right) &\\
            = & \sum_{e_q \in \mathcal{E}_H} \sum_{v_i \in \mathcal{V}} W_I \left(e_q\right)^\beta G\left(e_q\right) W_G \left(e_q\right)^\gamma \delta\left(v_i, e_q\right) \frac{w_I\left(v_i\right)^\alpha w_G\left(v_i\right)^\kappa}{\left\lvert e_q\right\rvert} f\left(v_i\right) &\\
            = & \sum_{v_i \in \mathcal{V}} \sum_{e_q \in \mathcal{E}_H} W_I \left(e_q\right)^\beta G\left(e_q\right) W_G \left(e_q\right)^\gamma \delta\left(v_i, e_q\right) \frac{w_I\left(v_i\right)^\alpha w_G\left(v_i\right)^\kappa}{\left\lvert e_q\right\rvert} f\left(v_i\right) &\\
            = & \sum_{v_i \in \mathcal{V}} w_I\left(v_i\right)^\alpha f\left(v_i\right) \sum_{e_q \in \mathcal{E}_H} \delta\left(v_i, e_q\right) \frac{w_G\left(v_i\right)^\kappa}{\left\lvert e_q\right\rvert} W_I \left(e_q\right)^\beta W_G \left(e_q\right)^\gamma G\left(e_q\right) &\\
            = & \sum_{v_i \in \mathcal{V}} w_I \left(v_i\right)^\alpha f\left(v_i\right) \nabla_v^* G\left(e_q\right) = {\langle f, \nabla^*_v G \rangle}_{\mathcal{H}\left(\mathcal{V}\right)} &\\
	\end{aligned}$\\

	Therefore, with the previous definition for the vertex adjoint operator $\nabla^*_v$, the equality ${\langle G, \nabla_v f \rangle}_{\mathcal{H}\left(\mathcal{E}_H\right)} = {\langle f, \nabla^*_v G \rangle}_{\mathcal{H}\left(\mathcal{V}\right)}$ holds true for all vertex functions $f \in \mathcal{H}\left(\mathcal{V}\right)$ and all hyperedge functions $G \in \mathcal{H}\left(\mathcal{E}_H\right)$.\\
\end{proof}



\begin{definition}[\textbf{Vertex $p$-Laplacian operator $\Delta_v^p$}]
	For an unoriented hypergraph $UH = \left(\mathcal{V}, \mathcal{E}_H\right)$ with vertex weight functions $w_I$ and $w_G$ and hyperedge weight functions $W_I$ and $W_G$, the vertex $p$-Laplacian operator $\Delta_v^p$ with parameters $\alpha, \beta, \gamma, \kappa \in \mathbb{R}$ is given by:
	{\small\begin{equation*}
		\Delta_v^p: ~ \mathcal{H}\left(\mathcal{V}\right) \longrightarrow \mathcal{H}\left(\mathcal{V}\right) \quad f \longmapsto \Delta_v^p f \quad \quad \quad
		\Delta_v^p f: ~ \mathcal{V} \longrightarrow \mathbb{R} \quad v_i \longmapsto \Delta_v^p f \left(v_i\right) =
	\end{equation*}
	\begin{equation*}
		\sum_{e_q \in \mathcal{E}_H} \delta\left(v_i, e_q\right) \frac{w_G \left(v_i\right)^\kappa}{\left\lvert e_q\right\rvert} W_I \left(e_q\right)^\beta W_G \left(e_q\right)^{p \gamma} \left\lvert\sum_{v_j \in \mathcal{V}} \delta\left(v_j, e_q\right) \frac{w_I \left(v_j\right)^\alpha w_G \left(v_j\right)^\kappa}{\left\lvert e_q\right\rvert} f\left(v_j\right)\right\rvert^{p - 2}
	\end{equation*}
	\begin{equation}
        \label{eq:p_laplace_hypergraph}
		\sum_{v_k \in \mathcal{V}} \delta\left(v_k, e_q\right) \frac{w_I \left(v_k\right)^\alpha w_G \left(v_k\right)^\kappa}{\left\lvert e_q\right\rvert} f\left(v_k\right).
	\end{equation}}
\end{definition}

\begin{theorem}[\textbf{Connection vertex gradient $\nabla_v$, vertex divergence $\mathrm{div}_v$, and vertex $p$-Laplacian $\Delta_v^p$}]
	For an unoriented hypergraph $UH = \left(\mathcal{V}, \mathcal{E}_H\right)$ with vertex weight functions $w_I$ and $w_G$ and hyperedge weight functions $W_I$ and $W_G$, the vertex $p$-Laplacian $\Delta_v^p$ fulfills the equality
	{\small\begin{equation}
		\Delta_v^p f = \mathrm{div}_v \left(\left\lvert \nabla_v f\right\rvert^{p - 2} \nabla_v f\right)
	\end{equation}}
	\hspace{-0.66em} for all vertex functions $f \in \mathcal{H}\left(\mathcal{V}\right)$.
\end{theorem}

\begin{proof}\ \\
	Given a weighted unoriented hypergraph $UH = \left(\mathcal{V}, \mathcal{E}_H, w, W\right)$ and a vertex function $f \in \mathcal{H}\left(\mathcal{V}\right)$, then the definitions of the vertex divergence operator $\text{div}_v$ and the vertex gradient operator $\nabla_v$ lead to the following for all vertices $v_i \in \mathcal{V}$:
	
	$\begin{aligned}[t]	
		& \text{div}_v \left(\left\lvert \nabla_v f\right\rvert^{p - 2} \nabla_v f\right)\left(v_i\right) &\\	
            = & \sum_{e_q \in \mathcal{E}_H} \delta\left(v_i, e_q\right) \frac{w_G \left(v_i\right)^\kappa}{\left\lvert e_q\right\rvert} W_I \left(e_q\right)^\beta W_G \left(e_q\right)^\gamma \left\lvert \nabla_v f\left(e_q\right)\right\rvert^{p - 2} \nabla_v f\left(e_q\right) &\\
		= & \sum_{e_q \in \mathcal{E}_H} \delta\left(v_i, e_q\right) \frac{w_G \left(v_i\right)^\kappa}{\left\lvert e_q\right\rvert} W_I \left(e_q\right)^\beta W_G \left(e_q\right)^\gamma &\\
		& \quad \quad \left\lvert W_G \left(e_q\right)^\gamma \sum_{v_j \in \mathcal{V}} \delta\left(v_j, e_q\right) \frac{w_I\left(v_j\right)^\alpha w_G\left(v_j\right)^\kappa}{\left\lvert e_q\right\rvert} f\left(v_j\right)\right\rvert^{p - 2} &\\
		& \quad \quad W_G \left(e_q\right)^\gamma \sum_{v_k \in \mathcal{V}} \delta\left(v_k, e_q\right) \frac{w_I\left(v_k\right)^\alpha w_G\left(v_k\right)^\kappa}{\left\lvert e_q\right\rvert} f\left(v_k\right) &\\
	\end{aligned}$\\
	
	Since the hyperedge weight function $W_G$ maps to positive values, the following reformulation holds true and leads to the vertex $p$-Laplacian definition:
	
	$\begin{aligned}[t]	
		= & \sum_{e_q \in \mathcal{E}_H} \delta\left(v_i, e_q\right) \frac{w_G \left(v_i\right)^\kappa}{\left\lvert e_q\right\rvert} W_I \left(e_q\right)^\beta W_G \left(e_q\right)^{2 \gamma + \gamma \left(p - 2\right)} &\\
		& \quad \quad \left\lvert \sum_{v_j \in \mathcal{V}} \delta\left(v_j, e_q\right) \frac{w_I\left(v_j\right)^\alpha w_G\left(v_j\right)^\kappa}{\left\lvert e_q\right\rvert} f\left(v_j\right)\right\rvert^{p - 2} &\\
		& \quad \quad \sum_{v_k \in \mathcal{V}} \delta\left(v_k, e_q\right) \frac{w_I\left(v_k\right)^\alpha w_G\left(v_k\right)^\kappa}{\left\lvert e_q\right\rvert} f\left(v_k\right) &\\
		= & \sum_{e_q \in \mathcal{E}_H} \delta\left(v_i, e_q\right) \frac{w_G \left(v_i\right)^\kappa}{\left\lvert e_q\right\rvert} W_I \left(e_q\right)^\beta W_G \left(e_q\right)^{\gamma p} &\\
		& \quad \quad \left\lvert \sum_{v_j \in \mathcal{V}} \delta\left(v_j, e_q\right) \frac{w_I\left(v_j\right)^\alpha w_G\left(v_j\right)^\kappa}{\left\lvert e_q\right\rvert} f\left(v_j\right)\right\rvert^{p - 2} &\\
		& \quad \quad \sum_{v_k \in \mathcal{V}} \delta\left(v_k, e_q\right) \frac{w_I\left(v_k\right)^\alpha w_G\left(v_k\right)^\kappa}{\left\lvert e_q\right\rvert} f\left(v_k\right) &\\
		= & ~ \Delta_v^p f \left(v_i\right) &\\
	\end{aligned}$\\
	
	Therefore, using the previously introduced definitions for the vertex gradient $\nabla_v$, the vertex divergence $\text{div}_v$, and the vertex $p$-Laplacian $\Delta_v^p$ shows that the equality $\Delta_v^p f\left(v_i\right) = \text{div}_v \left(\left\lvert \nabla_v f\right\rvert^{p - 2} \nabla_v f\right) \left(v_i\right)$ holds true for all vertices $v_i \in \mathcal{V}$ and for all vertex functions $f \in \mathcal{H}\left(\mathcal{V}\right)$.\\
\end{proof}












\begin{definition}[\textbf{Image to vectors}]\\
    Suppose a $n \times m$ image $I$ with $n m$ pixels $p_{r s}$ for $r \in \left\{1, 2, \dots n\right\}$ and $s \in \left\{1, 2, \dots m\right\}$ is given, where each pixel has a gray value $p_{r s} \in \left[0, 1\right]$.\\

    For each pixel $p_{r s}$ we define a vector $x_{r s} \in \left[0, 1\right]^{{\left(2b + 1\right)}^2}$ including information about the ${\left(2b + 1\right)}^2 - 1$ local neighbors of $p_{r s}$ with ${\left(2b + 1\right)}^2$ denoting the batch size:

    \begin{tabular}{cc}
        \begin{minipage}{0.55\textwidth}
            \hspace{-0.75cm}
            \setlength{\unitlength}{\dimensiona}
            \begin{tikzpicture}(0,0)
                \put (0,8.6) {\pixela}
                \put (1,8.6) {\pixela}
                \put (2,8.6) {\pixela}
                \put (3,8.6) {\pixela}
                \put (4,8.6) {\pixela}
                \put (5,8.6) {\pixela}
                \put (0,4.6) {\pixela}
                \put (1,4.6) {\pixela}
                \put (2,4.6) {\pixela}
                \put (3,4.6) {\pixela}
                \put (4,4.6) {\pixela}
                \put (5,4.6) {\pixela}
                \put (0,7.6) {\pixela}
                \put (1,7.6) {\pixela}
                \put (2,7.6) {\pixela}
                \put (3,7.6) {\pixela}
                \put (4,7.6) {\pixela}
                \put (5,7.6) {\pixela}
                \put (0,6.6) {\pixela}
                \put (1,6.6) {\pixela}
                \put (2,6.6) {\pixela}
                \put (3,6.6) {\pixela}
                \put (4,6.6) {\pixela}
                \put (5,6.6) {\pixela}
                \put (0,5.6) {\pixela}
                \put (1,5.6) {\pixela}
                \put (2,5.6) {\pixela}
                \put (3,5.6) {\pixela}
                \put (4,5.6) {\pixela}
                \put (5,5.6) {\pixela}
                \put (0,4.6) {\pixela}
                \put (1,4.6) {\pixela}
                \put (2,4.6) {\pixela}
                \put (3,4.6) {\pixela}
                \put (4,4.6) {\pixela}
                \put (5,4.6) {\pixela}
                \put (0,3.6) {\pixela}
                \put (1,3.6) {\pixela}
                \put (2,3.6) {\pixela}
                \put (3,3.6) {\pixela}
                \put (4,3.6) {\pixela}
                \put (5,3.6) {\pixela}
                \node (v11) at (0.6,11.2) {\small{$p_{\substack{r - b, \\ s - b}}$}};
                \node (v12) at (1.9,11.2) {\small{$p_{\substack{r - b, \\ s - b + 1}}$}};
                \node (v14) at (4.3,11.2) {\small{$\dots$}};
                \node (v16) at (6.75,11.2) {\small{$p_{\substack{r - b, \\ s + b}}$}};
                \node (v21) at (0.65,9.95) {\small{$p_{\substack{r - b + 1, \\ s - b}}$}};
                \node (v22) at (1.85,9.95) {\small{$p_{\substack{r - b + 1, \\ s - b + 1}}$}};
                \node (v24) at (4.3,9.95) {\small{$\dots$}};
                \node (v26) at (6.75,9.95) {\small{$p_{\substack{r - b + 1, \\ s + b}}$}};
                \node (v41) at (0.6,7.6) {\small{$\vdots$}};
                \node (v42) at (1.8,7.6) {\small{$\vdots$}};
                \node (v44) at (4.3,7.5) {\small{$p_{r s}$}};
                \node (v46) at (6.75,7.6) {\small{$\vdots$}};
                \node (v61) at (0.6,5) {\small{$p_{\substack{r + b, \\ s - b}}$}};
                \node (v62) at (1.9,5) {\small{$p_{\substack{r + b, \\ s - b + 1}}$}};
                \node (v64) at (4.3,5) {\small{$\dots$}};
                \node (v66) at (6.75,5) {\small{$p_{\substack{r + b, \\ s + b}}$}};
            \end{tikzpicture}
        \end{minipage}
        \begin{minipage}{0.45\textwidth}
            \begin{equation}
        x_{r s} = \left(
            \begin{array}{c}
            p_{r - b, ~ s - b}\\
            p_{r - b, ~ s - b + 1}\\
            \vdots\\
            p_{r - b, ~ s + b}\\
            p_{r - b + 1, ~ s - b}\\
            p_{r - b + 1, ~ s - b + 1}\\
            \vdots\\
            p_{r - b + 1, ~ s + b}\\
            \vdots\\
            p_{r s}\\
            \vdots\\
            p_{r + b, ~ s - b}\\
            p_{r + b, ~ s - b + 1}\\
            \vdots\\
            p_{r + b, ~ s + b}\\
            \end{array}
        \right)
            \end{equation}
        \end{minipage}
    \end{tabular}

    In the case of $r + y \notin \left\{1, 2, \dots n\right\}$ for $y \in \left\{-b, -b + 1, \dots, b - 1, b\right\}$, or $s + z \notin \left\{1, 2, \dots m\right\}$ for $z \in \left\{-b, -b + 1, \dots, b - 1, b\right\}$ we define the vector entry $p_{r + y, ~ s + z}$ as

    \begin{equation}
        p_{r + y, ~ s + z} = \left\{
            \begin{array}{ll}
			p_{1, ~ s + z} & \quad \text{Top edge:} ~ r + y < 1, ~ s + z \in \left\{1, 2, \dots m\right\} \\
                p_{1, ~ m} & \quad \text{Top right corner:} ~ r + y < 1, ~ m < s + z \\
                p_{r + y, ~ m} & \quad \text{Right edge:} ~ r + y \in \left\{1, 2, \dots n\right\}, ~ m < s + z \\
                p_{n, m} & \quad \text{Bottom right corner:} ~ n < r + y, ~ m < s + z \\
                p_{n, ~ s + z} & \quad \text{Bottom edge:} ~ n < r + y, ~ s + z \in \left\{1, 2, \dots m\right\} \\
                p_{n, ~ 1} & \quad \text{Bottom left corner:} ~ n < r + y, ~ s + z < 1 \\
			p_{r + y, ~ 1} & \quad \text{Left edge:} ~ r + y \in \left\{1, 2, \dots n\right\}, ~ s + z < 1 \\
                p_{1, ~ 1} & \quad \text{Top left corner:} ~ r + y < 1, ~ s + z < 1
		\end{array}
        \right.
            \end{equation}
\end{definition}

\begin{definition}[\textbf{Vectors to (un)oriented hypergraph}]\\
    Given a set of vectors $\left\{x_{r s} ~ \middle| ~ r  \in \left\{1, 2, \dots n\right\}, s \in \left\{1, 2, \dots m\right\}\right\}$ representing a $n \times m$ Image $I$, we define the $k$-nearest neighbor oriented hypergraph $OH_k = \left(\mathcal{V}, \mathcal{A}_H\right)$ for $k \in \mathbb{N}_{> 0}$ as:
    
    \begin{equation}
        \mathcal{V} = \left\{p_{r s} ~ \middle| ~ r \in \left\{1, 2, \dots n\right\}, s \in \left\{1, 2, \dots m\right\}\right\}
    \end{equation}
    \begin{equation}
        \mathcal{A}_H = \left\{\left(V_k\left(p_{r s}\right), \left\{p_{r s}\right\}\right) ~ \middle| ~ r \in \left\{1, 2, \dots n\right\}, s \in \left\{1, 2, \dots m\right\}\right\}
    \end{equation}
    
    with $V_k\left(p_{r s}\right) = \left\{p_{t u} \in \mathcal{V} \backslash\left\{p_{r s}\right\} ~ \middle| ~ \exists p_{\tilde{t} \tilde{u}} \in V: \lvert\lvert x_{r s} - x_{t u}\rvert\rvert_2 \leq \lvert\lvert x_{r s} - x_{\tilde{t} \tilde{u}}\rvert\rvert_2 \right\}$, where $V := \argmin_{V \subset \mathcal{V} \backslash\left\{p_{r s}\right\}, ~ \left\lvert V\right\rvert = k} \left\{\sum_{p_{\tilde{t} \tilde{u}} \in V} \lvert\lvert x_{r s} - x_{\tilde{t} \tilde{u}}\rvert\rvert_2\right\}$. The set $V_k\left(p_{r s}\right)$ consists of the (at least) $k$ nearest pixels $p_{t u} \in \mathcal{V} \backslash \left\{p_{r s}\right\}$ of $p_{r s}$, where distance is measured as the level of similarity of the local neighborhood of the respective pixels $p_{r s}$ and $p_{t u}$.

    In order to obtain an unoriented hypergraph from a given $n \times m$ image $I$, we define the $\epsilon$-neighborhood unoriented hypergraph $UH_\epsilon = \left(\mathcal{V}, \mathcal{E}_H\right)$ for $\epsilon > 0$ as:

    \begin{equation}
        \mathcal{V} = \left\{p_{r s} ~ \middle| ~ r \in \left\{1, 2, \dots n\right\}, s \in \left\{1, 2, \dots m\right\}\right\}
    \end{equation}
    \begin{equation}
        \mathcal{E}_H = \left\{V_\epsilon\left(p_{r s}\right) ~ \middle| ~ r \in \left\{1, 2, \dots n\right\}, s \in \left\{1, 2, \dots m\right\}, \left\lvert V_\epsilon\left(p_{r s}\right)\right\rvert \geq 2\right\}
    \end{equation}

    where $V_\epsilon\left(p_{r s}\right) = \left\{p_{t u} \in \mathcal{V} ~ \middle| ~ \lvert\lvert x_{r s} - x_{t u}\rvert\rvert_2 < \epsilon\right\}$ contains all pixels $p_{t u}$ in the $\epsilon$ neighborhood of $p_{r s}$, where the distance is again measured as the level of similarity of the local neighborhoods. Note that $p_{r s} \in V_\epsilon\left(p_{r s}\right)$ for all $r \in \left\{1, 2, \dots n\right\}, s \in \left\{1, 2, \dots m\right\}$ and $\epsilon > 0$. Hence, we require $\left\lvert V_\epsilon\left(p_{r s}\right)\right\rvert \geq 2$ so that we only consider hyperedges, which connect at least two pixels.
\end{definition}

\begin{remark}
    Encoding an image $I$ as a hypergraph based on the $k$-nearest neighbor principle results in an oriented hypergraph, because $p_{t u} \in V_k\left(p_{r s}\right) \quad \Longrightarrow \quad \exists V \subset \mathcal{V}: \left\lvert V\right\rvert = k, p_{t u} \in V ~ \text{and} ~ \sum_{p_{\tilde{t} \tilde{u}} \in V} \lvert\lvert x_{r s} - x_{\tilde{t} \tilde{u}}\rvert\rvert_2 = \min_{V \subset \mathcal{V} \backslash\left\{p_{r s}\right\}, ~ \left\lvert V\right\rvert = k} \left\{\sum_{p_{\tilde{t} \tilde{u}} \in V} \lvert\lvert x_{r s} - x_{\tilde{t} \tilde{u}}\rvert\rvert_2\right\}$ (the $\argmin$ is not necessarily unique). However, this does not imply $p_{r s} \in V_k\left(p_{t u}\right)$, because there could exist $p_{t_1 u_1}, p_{t_2 u_2}, \dots p_{t_k u_k} \in \mathcal{V} \backslash \left\{p_{r s}\right\}$ such that: $\lvert\lvert x_{t_1 u_1} - x_{t u}\rvert\rvert_2, \lvert\lvert x_{t_2 u_2} - x_{t u}\rvert\rvert_2, \dots \lvert\lvert x_{t_k u_k} - x_{t u}\rvert\rvert_2 <  \lvert\lvert x_{r s} - x_{t u}\rvert\rvert_2$ and therefore, $p_{r s}$ would not be part of any $V$ with $V \in \argmin_{V \subset \mathcal{V} \backslash\left\{p_{t u}\right\}, ~ \left\lvert V\right\rvert = k} \left\{\sum_{p_{\tilde{t} \tilde{u}} \in V} \lvert\lvert x_{t u} - x_{\tilde{t} \tilde{u}}\rvert\rvert_2\right\}$.\\

    In contrast to this, considering $\epsilon$-neighborhoods leads to an unoriented hypergraph, because $p_{t u} \in V_\epsilon\left(p_{r s}\right) \backslash \left\{p_{r s}\right\} \quad \Longrightarrow \quad \lvert\lvert x_{r s} - x_{t u}\rvert\rvert_2 < \epsilon \quad \Longrightarrow \quad \lvert\lvert x_{t u} - x_{r s}\rvert\rvert_2 < \epsilon \quad \Longrightarrow \quad p_{r s} \in V_\epsilon\left(p_{t u}\right) \backslash \left\{p_{t u}\right\}$.
\end{remark}



\begin{definition}[\textcolor{arifaz}{\textbf{Image to vectors}}]\\
    Suppose a $n \times m$ image $I$ with $n m$ pixels $p_{r s}$ for $r \in \left\{1, 2, \dots n\right\}$ and $s \in \left\{1, 2, \dots m\right\}$ is given, where each pixel has a gray value $p_{r s} \in \left[0, 1\right]$.\\

    Then instead of investigating the similarity of singular pixels, we want to investigate similarity in a local neighborhood and thus for a patch size $p \in \left\{1, 4, 9, 16, 25, \dots \min\left\{n, m\right\}^2\right\}$, we can define patches $x_{u w}$ for $u \in \left\{1, 2, \dots n - \sqrt{p} + 1\right\}$ and $w \in \left\{1, 2, \dots m - \sqrt{p} + 1\right\}$:

    \begin{tabular}{cc}
        \begin{minipage}{0.55\textwidth}
            \vspace{1.4cm}
            \hspace{-0.75cm}
            \setlength{\unitlength}{\dimensionb}
            \begin{tikzpicture}(0,0)
                \put (0,4.6) {\pixelb}
                \put (1,4.6) {\pixelb}
                \put (2,4.6) {\pixelb}
                \put (3,4.6) {\pixelb}
                \put (4,4.6) {\pixelb}
                \put (0,7.6) {\pixelb}
                \put (1,7.6) {\pixelb}
                \put (2,7.6) {\pixelb}
                \put (3,7.6) {\pixelb}
                \put (4,7.6) {\pixelb}
                \put (0,6.6) {\pixelb}
                \put (1,6.6) {\pixelb}
                \put (2,6.6) {\pixelb}
                \put (3,6.6) {\pixelb}
                \put (4,6.6) {\pixelb}
                \put (0,5.6) {\pixelb}
                \put (1,5.6) {\pixelb}
                \put (2,5.6) {\pixelb}
                \put (3,5.6) {\pixelb}
                \put (4,5.6) {\pixelb}
                \put (0,4.6) {\pixelb}
                \put (1,4.6) {\pixelb}
                \put (2,4.6) {\pixelb}
                \put (3,4.6) {\pixelb}
                \put (4,4.6) {\pixelb}
                \put (0,3.6) {\pixelb}
                \put (1,3.6) {\pixelb}
                \put (2,3.6) {\pixelb}
                \put (3,3.6) {\pixelb}
                \put (4,3.6) {\pixelb}
                \node (v11) at (0.7,11.4) {\small{$p_{u w}$}};
                \node (v13) at (3.55,11.35) {\small{$\dots$}};
                \node (v15) at (6.35,11.35) {\small{$p_{\substack{u, \\ w + \sqrt{p} - 1}}$}};
                \node (v31) at (0.7,8.65) {\small{$\vdots$}};
                \node (v33) at (3.55,8.65) {\small{$\ddots$}};
                \node (v35) at (6.35,8.65) {\small{$\vdots$}};
                \node (v61) at (0.7,5.8) {\small{$p_{\substack{u + \sqrt{p} - 1, \\ w}}$}};
                \node (v64) at (3.55,5.8) {\small{$\dots$}};
                \node (v66) at (6.35,5.75) {\small{$p_{\substack{u + \sqrt{p} - 1, \\ w + \sqrt{p} - 1}}$}};
            \end{tikzpicture}
            \vspace{0.5cm}
        \end{minipage}
        \begin{minipage}{0.45\textwidth}
            \begin{equation}
        x_{u w} = \left(
            \begin{array}{c}
            p_{u w}\\
            p_{u, ~ w + 1}\\
            \vdots\\
            p_{u, ~ w + \sqrt{p} - 1}\\
            p_{u + 1, ~ w}\\
            p_{u + 1, ~ w + 1}\\
            \vdots\\
            p_{u + 1, ~ w + \sqrt{p} - 1}\\
            \vdots\\
            p_{r + \sqrt{p} - 1, ~ w}\\
            p_{r + \sqrt{p} - 1, ~ w + 1}\\
            \vdots\\
            p_{r + \sqrt{p} - 1, ~ w + \sqrt{p} - 1}\\
            \end{array}
        \right)
            \end{equation}
        \end{minipage}
    \end{tabular}
\end{definition}

\begin{definition}[\textcolor{arifaz}{\textbf{Vectors to (un)oriented hypergraph}}]\\
    Given a set of vectors $\left\{x_{u w} ~ \middle| ~ u  \in \left\{1, 2, \dots n - \sqrt{p} + 1\right\}, s \in \left\{1, 2, \dots m - \sqrt{p} + 1\right\}\right\}$ representing a $n \times m$ Image $I$, we define the $k$-nearest neighbor oriented hypergraph $OH_k = \left(\mathcal{V}, \mathcal{A}_H\right)$ for $k \in \mathbb{N}_{> 0}$ as:
    
    \begin{equation}
        \mathcal{V} = \left\{x_{u w} ~ \middle| ~ u \in \left\{1, 2, \dots n - \sqrt{p} + 1\right\}, w \in \left\{1, 2, \dots m - \sqrt{p} + 1\right\}\right\}
    \end{equation}
    \begin{equation}
        \mathcal{A}_H = \left\{\left(V_k\left(x_{u w}\right), \left\{x_{u w}\right\}\right) ~ \middle| ~ u \in \left\{1, 2, \dots n - \sqrt{p} + 1\right\}, s \in \left\{1, 2, \dots m - \sqrt{p} + 1\right\}\right\}
    \end{equation}
    
    with $V_k\left(x_{u w}\right) = \left\{x_{y z} \in \mathcal{V} \backslash\left\{x_{u w}\right\} ~ \middle| ~ \exists x_{\tilde{y} \tilde{z}} \in V: \lvert\lvert x_{u w} - x_{y z}\rvert\rvert_2 \leq \lvert\lvert x_{u w} - x_{\tilde{y} \tilde{z}}\rvert\rvert_2 \right\}$, where $V := \argmin_{V \subset \mathcal{V} \backslash\left\{x_{u w}\right\}, ~ \left\lvert V\right\rvert = k} \left\{\sum_{x_{\tilde{y} \tilde{z}} \in V} \lvert\lvert x_{u w} - x_{\tilde{y} \tilde{z}}\rvert\rvert_2\right\}$. The set $V_k\left(x_{u w}\right)$ consists of the (at least) $k$ nearest patches $x_{y z} \in \mathcal{V} \backslash \left\{x_{u w}\right\}$ of $x_{u w}$, where distance is measured as the level of similarity.

    In order to obtain an unoriented hypergraph from a given $n \times m$ image $I$, we define the $\epsilon$-neighborhood unoriented hypergraph $UH_\epsilon = \left(\mathcal{V}, \mathcal{E}_H\right)$ for $\epsilon > 0$ as:

    \begin{equation}
        \mathcal{V} = \left\{x_{u w} ~ \middle| ~ u \in \left\{1, 2, \dots n - \sqrt{p} + 1\right\}, w \in \left\{1, 2, \dots m - \sqrt{p} + 1\right\}\right\}
    \end{equation}
    \begin{equation}
        \mathcal{E}_H = \left\{V_\epsilon\left(x_{u w}\right) ~ \middle| ~ u \in \left\{1, 2, \dots n - \sqrt{p} + 1\right\}, w \in \left\{1, 2, \dots m - \sqrt{p} + 1\right\}, \left\lvert V_\epsilon\left(x_{u w}\right)\right\rvert \geq 2\right\}
    \end{equation}

    where $V_\epsilon\left(x_{u w}\right) = \left\{x_{y z} \in \mathcal{V} ~ \middle| ~ \lvert\lvert x_{u w} - x_{y z}\rvert\rvert_2 < \epsilon\right\}$ contains all patches $x_{y z}$ in the $\epsilon$ neighborhood of $x_{u w}$, where the distance is again measured as the level of similarity. Note that $x_{u w} \in V_\epsilon\left(x_{u w}\right)$ for all $u \in \left\{1, 2, \dots n - \sqrt{p} + 1\right\}, w \in \left\{1, 2, \dots m - \sqrt{p} + 1\right\}$ and $\epsilon > 0$. Hence, we require $\left\lvert V_\epsilon\left(x_{u w}\right)\right\rvert \geq 2$ so that we only consider hyperedges, which connect at least two patches.
\end{definition}

\begin{remark}
    Encoding an image $I$ as a hypergraph based on the $k$-nearest neighbor principle results in an oriented hypergraph, because $x_{y z} \in V_k\left(x_{u w}\right) \quad \Longrightarrow \quad \exists V \subset \mathcal{V}: \left\lvert V\right\rvert = k, x_{y z} \in V ~ \text{and} ~ \sum_{p_{\tilde{y} \tilde{z}} \in V} \lvert\lvert x_{u w} - x_{\tilde{y} \tilde{z}}\rvert\rvert_2 = \min_{V \subset \mathcal{V} \backslash\left\{x_{u w}\right\}, ~ \left\lvert V\right\rvert = k} \left\{\sum_{p_{\tilde{y} \tilde{z}} \in V} \lvert\lvert x_{u w} - x_{\tilde{y} \tilde{z}}\rvert\rvert_2\right\}$ (the $\argmin$ is not necessarily unique). However, this does not imply $x_{u w} \in V_k\left(x_{y z}\right)$, because there could exist $x_{x_1 y_1}, p_{x_2 y_2}, \dots p_{x_k y_k} \in \mathcal{V} \backslash \left\{x_{u w}\right\}$ such that: $\lvert\lvert x_{y_1 z_1} - x_{y z}\rvert\rvert_2, \lvert\lvert x_{y_2 z_2} - x_{y z}\rvert\rvert_2, \dots \lvert\lvert x_{y_k z_k} - x_{y z}\rvert\rvert_2 <  \lvert\lvert x_{u w} - x_{y z}\rvert\rvert_2$ and therefore, $x_{y z}$ would not be part of any $V$ with $V \in \argmin_{V \subset \mathcal{V} \backslash\left\{x_{y z}\right\}, ~ \left\lvert V\right\rvert = k} \left\{\sum_{p_{\tilde{y} \tilde{z}} \in V} \lvert\lvert x_{y z} - x_{\tilde{y} \tilde{z}}\rvert\rvert_2\right\}$.\\

    In contrast to this, considering $\epsilon$-neighborhoods leads to an unoriented hypergraph, because $x_{y z} \in V_\epsilon\left(x_{u w}\right) \backslash \left\{x_{u w}\right\} \quad \Longrightarrow \quad \lvert\lvert x_{u w} - x_{y z}\rvert\rvert_2 < \epsilon \quad \Longrightarrow \quad \lvert\lvert x_{y z} - x_{u w}\rvert\rvert_2 < \epsilon \quad \Longrightarrow \quad x_{u w} \in V_\epsilon\left(x_{y z}\right) \backslash \left\{x_{y z}\right\}$.
\end{remark}
